Multi-headed Neural Ensemble Search

Ensembles of CNN models trained with different seeds (also known as Deep Ensembles) are known to achieve superior performance over a single copy of the CNN. Neural Ensemble Search (NES) can further boost performance by adding architectural diversity. However, the scope of NES remains prohibitive under limited computational resources. In this work, we extend NES to multi-headed ensembles, which consist of a shared backbone attached to multiple prediction heads. Unlike Deep Ensembles, these multi-headed ensembles can be trained end to end, which enables us to leverage one-shot NAS methods to optimize an ensemble objective. With extensive empirical evaluations, we demonstrate that multi-headed ensemble search finds robust ensembles 3 times faster, while having comparable performance to other ensemble search methods, in both predictive performance and uncertainty calibration.

==> Multihead NES/content/abstract.tex <==
Ensembles of CNN models trained with different seeds (also known as Deep Ensembles) are known to achieve superior performance over a single copy of the CNN.
%, especially in terms of uncertainty estimates.
Neural Ensemble Search (NES) can further boost performance by adding architectural diversity.
%optimizing an ensemble objective. 
However, 
%due to inherently large training overhead of Deep Ensembles, 
the scope of NES remains prohibitive under limited computational resources.
In this work, we extend NES to multi-headed ensembles, which consist of a shared backbone attached to multiple prediction heads. 
Unlike Deep Ensembles, these multi-headed ensembles can be trained end to end, which enables us to leverage one-shot NAS methods to optimize an ensemble objective. With extensive empirical evaluations, we demonstrate that multi-headed ensemble search finds robust ensembles $3\times$ faster, while having comparable performance to other ensemble search methods, in both predictive performance and uncertainty calibration.

% Ensembles of neural networks are known to achieve superior performance over single networks.
% In conventional CNN ensembles (also known as Deep Ensembles) each member is trained independently before their predictions are combined. While this is effective, Deep Ensembles can be computationally intensive --- during training, as well as, inference. 
% Due to its training overhead, the scope of ensemble optimization methods remain prohibitive under limited computational resources. 
% An efficient alternative to Deep Ensembles are multi-headed ensembles, which consist of a shared backbone attached to multiple prediction heads. In this work, we focus on searching for optimal prediction head architectures in a multi-headed setting through one-shot NAS methods. 
% % Unlike Deep Ensembles, multi-headed models are trained end to end, which enables us to extend one-shot NAS methods to optimize an ensemble objective. 
% With extensive empirical evaluation, we demonstrate that multi-headed ensemble search finds robust ensembles $3\times$ faster, while having comparable performance to other ensemble search methods, in both predictive performance and uncertainty calibration.


==> Multihead NES/content/body.tex <==

\section{Introduction}

Ensembles of neural networks are a common solution to improve predictive performance and uncertainty calibration \citep{hansen1990neural}. Ensembles of networks trained with different random initializations (known as \emph{Deep Ensembles}) can lead to well-performing and diverse models as they include different local optima \citep{lakshminarayanan2016simple, fort2019deep}.
They have also been shown to outperform approximate Bayesian methods \citep{lakshminarayanan2016simple, ovadia2019trust, gustafsson2020evaluating}.
On top of that, Neural Ensemble Search (NES)~\citep{zaidi2020neural} and HyperDeepEns~\citep{wenzel2021hyperparameter} can further improve performance by searching for a complementary set of ensemble members.
However, building and maintaining multiple models can be expensive.
%, more so, for ensemble search methods.

While more efficient alternatives have been proposed for constructing ensembles, such as BatchEnsembles \citep{wen2020batchensemble} and Snapshot Ensembles \citep{huang2017snapshot,loshchilov2017sgdr}, they do not typically outperform deep ensembles. Multi-headed networks are another means to build efficient ensembles which uses a single shared backbone with multiple prediction heads \citep{lee2015m, lan2018knowledge}. 
% \tct{
While multi-headed models have been studied before, to the best of our knowledge, there is no prior work that studies the performance impact of searching head architectures.
%or w.r.t. model calibration. 
%In this work, we formulate head architecture search in multi-headed models as a NAS problem. 
In this work, we employ neural architecture search (NAS)~\citep{elsken2019neural} to search for the heads' architecture in the multi-headed models.
Unlike Deep Ensembles, multi-headed models are trained end-to-end, which allows one-shot NAS methods \citep{bender2018understanding, liu2019darts} to optimize an ensemble objective.

\begin{table}[t]
    \centering
    \caption{ Overview: Multi-headed NES (MH-NES) leads to performant models on CIFAR-100 with significantly less search costs. }
    \vspace{2mm}
	{%\scriptsize
	\resizebox{1.0\linewidth}{!}{
	\begin{tabular}{lcccc}
	\toprule
	\textbf{Method} & \textbf{\# Params} & \textbf{Search Cost} & \textbf{Error} & \textbf{ECE} \\
					& \textbf{(M)} 			& \textbf{(GPU hours)} & & \\
	\midrule
	NES-RS & 4.0 & 15.2 & 19.75{\tiny$\pm$0.27} & 0.021{\tiny$\pm$0.001} \\
	HyperDeepEns (RS) & 4.2 & 28.7 & 20.11{\tiny$\pm$0.18} & 0.019{\tiny$\pm$0.003} \\
	MH-NES & \textbf{2.7} & \textbf{5.0} & \textbf{19.65{\tiny$\pm$0.09}} & \textbf{0.017{\tiny$\pm$0.001}} \\
	\bottomrule
	\end{tabular}
	}
	}
    \label{tab:EX:ens_cost_teaser}
\end{table}

% \todo{FH: Could Table \ref{tab:EX:ens_cost_teaser} also include a measure of predictive uncertainty?}

The key contributions of this paper are as follows: 
\begin{itemize}
\itemsep 0pt\topsep-6pt\partopsep-6pt
%\denselist
    \item We extend the standard NAS search space to sample prediction heads in multi-headed ensembles. 
    \item We evaluate three one-shot NAS methods and demonstrate comparable or better performance to other ensemble search methods such as NES and HyperDeepEns, with significantly less search costs (see \autoref{tab:EX:ens_cost_teaser}).
    \item We provide an analysis and shed some light on potential factors affecting the performance of one-shot NAS methods in the multi-headed setting, particularly for larger ensemble sizes.
\end{itemize}
%\textbf{(1)} we extend the standard NAS search space to sample prediction heads in multi-headed ensembles. \textbf{(2)} We evaluate three one-shot NAS methods and demonstrate comparable or better performance to other ensemble search methods such as NES and HyperDeepEns, with significantly less search costs (see \autoref{tab:EX:ens_cost_teaser}). \textbf{(3)} We provide an analysis and shed some light on potential factors affecting the performance of one-shot NAS methods in the multi-headed setting, particularly for larger ensemble sizes.

%\begin{enumerate} 
    %\item We extend the standard NAS differentiable search space to sample prediction heads for multi-headed ensembles. 
    % \tct{Maybe you can say: we extend the standard NAS search space for MH models.}
    % \item We introduce a diversity encouraging loss to improve architecture search performance and evaluate different one-shot NAS methods to search for the optimal head configurations. \tct{Is this claim important since you finally say one-shot NAS doesn't work that well? I would remove it.}
    %\item We evaluate three one-shot NAS methods and demonstrate comparable performance to other ensemble search methods such as NES and HyperDeepEns.
    %\item We identify that random search-based methods outperform gradient-based one-shot NAS methods for larger ensembles and shed some light on potential factors affecting the search on multi-headed ensembles.
    % \tct{We evaluated three one-shot NAS methods and found ..... We shed some light on potential factors affecting the performance of one-shot NAS methods for ensembles. (maybe also mention that we can match the performance of NES/HyperDeepENs)}
%\end{enumerate}

% \textbf{(1)} ... list main highlights here.}

%Moreover, the joint training of all ensemble members allows for ensemble-aware or specialized terms in the objective.

%In this work, we design multi-headed ensembles with varying head architectures for strong ensemble performance.
%The difference in head architectures leads to more diverse predictions and better uncertainty calibration without having to introduce additional diversity constraints.
%However, choosing the head architectures is not straight-forward. AutoML \citep{hutter2019automated} and Neural Architecture Search (NAS) \citep{elsken2019neural} promises to relieve us from manually identifying well-performing heads that work together.
%One-shot architecture search \citep{bender2018understanding, liu2019darts} especially has shown good performance on conventional NAS problems and managed to remain computationally efficient.
%We use three one-shot architecture search methods: PC-DARTS \citep{xu2019pc}, DrNAS \citep{chen2021drnas} and RandomNAS \citep{li2020random} to identify heads that perform well together in a multi-headed network and provide strong ensemble performance.

% --------------------------------------------------------------------

\subsection{Related Work}

%\textbf{Ensembling} to boost model performance has been around for a long time \citep{hansen1990neural, dietterich2000ensemble}.
\textbf{Ensemble} methods~\citep{hansen1990neural, dietterich2000ensemble} are extensively used in machine learning research, as both a means to boost performance, but also for better calibration and uncertainty estimates of deep neural networks~\citep{lakshminarayanan2016simple}.
%Common ensembling methods for neural networks include training random initializations of parameters \citep{lakshminarayanan2016simple}, boosting \citep{moghimi2016boosted} and using checkpoints while training a network \citep{huang2017snapshot}.
Diversity in the predictions made by the ensemble base learners is believed to be crucial in order to obtain good ensembles. Some methods induce diversity by training with specialized losses \citep{lee2015m, zhou2018diverse}, building ensemble members with different topologies \citep{zaidi2020neural} or different training hyperparameters \citep{wenzel2021hyperparameter} to improve ensemble performance.
Multi-head networks trained under a unified objective can produce robust ensembles too, by utilizing diversity encouraging specialized losses \citep{lee2015m}, co-distillation \citep{lan2018knowledge} or both \citep{dvornik2019diversity}. 
%can be utilized to further improve the ensembles. 
% \cite{lan2018knowledge} proposed a co-distillation framework \citep{hinton2015distilling} using multi-headed architectures. 
% \citep{dvornik2019diversity} combined both co-distillation and diversity encouraging losses to build ensembles for few-shot learning.
% Most works on multi-headed ensembles have uniform head architectures. Model calibration in multi-headed ensembles has not been explored either.

%\textbf{Neural Architecture Search} (NAS) is the process of searching for an optimal neural network topology \citep{elsken2019neural}. 
\textbf{Neural Architecture Search} (NAS) aims to find an optimal neural network architecture that optimizes some objective (e.g. validation loss)~\citep{elsken2019neural}.
%Existing strategies using Bayesian optimization \citep{snoek2012practical}, 
Early methods, such as reinforcement learning \citep{zoph2016neural} and evolutionary algorithms \citep{real2019regularized}, but also more recent efficient methods~\citep{bender2018understanding, elsken2017simple, cai2019proxylessnas, liu2019darts, xu2019pc, chen2021drnas} have shown that NAS can find architectures that can surpass hand-crafted ones.
% DARTS \citep{liu2019darts} introduces a differentiable framework to search for architectures within a short period of time.
% Several future works improved the stability and efficiency of NAS methods, leading to better performance \citep{xu2019pc, chen2020progressive, chen2021drnas}.
Recently, NAS has also been applied to ensemble learning. Neural Ensemble Search (NES) \citep{zaidi2020neural} builds a pool of strong independent models with different architectures and applies ensemble selection to create the ensembles. On the other hand, AdaNAS~\citep{macko2019improving} iteratively adds base learners to an ensemble to improve the ensemble performance.
%
%This work has a similar motivation to NES \citep{zaidi2020neural}. 
%Our work is closely related to NES~\citep{zaidi2020neural}. 
While NES and AdaNAS construct ensembles by independently training the base learners, which is computationally expensive, we focus on multi-headed ensembles that are cheaper to construct and allow us to leverage efficient NAS methods to design their topology.

% --------------------------------------------------------------------

\section{Background}

\subsection{Multi-headed Ensembles}

Figure \ref{fig:BG:mh_arch} depicts an overview of a multi-headed ensemble for a classification task. The network can be divided into two sections: a \textit{lower block} shared by all the heads and \textit{multi-head block} consisting of $M$ heads. Each head may have similar or different architectures.

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/multi_head_arch.pdf}
    \caption{A multi-head ensemble for a CNN classifier}
    \label{fig:BG:mh_arch}
\end{figure}

Given a classification task, let $\gD_{train} = \{(x_n, y_n) : n = 1,...,N \} $ be the training set, where $x_n \in \sR^D$ is the $D$-dimensional input and $y_n \in \{1,..., C\}$ is the label, assumed to be one of the $C$ classes.
We denote a base learner, in our case neural networks, by $f_\theta$, where $\theta$ represents the network parameters. A network takes the input $x_i$ and outputs a vector of probabilistic class posteriors over the classes as $f_\theta(x) \in \sR^C$.
We construct an ensemble $F$ of $M$ members $f_{\theta_1}, ..., f_{\theta_M}$ by averaging the output of the networks. 

Let $\ell$ be the cost function. 
%An \textit{ensemble-aware loss} (Equation \ref{eq:BG:mh_loss}), is used during training. It 
We use an \emph{ensemble-aware loss function}, which includes the ensemble loss term, in addition to the individual head losses to improve the model performance:

\begin{equation}
    \gL_{train} = \sum_{i=1}^{M}{\ell(f_i(x), y)} + \ell(F(x), y).
    \label{eq:BG:mh_loss}
\end{equation}

\subsection{Differentiable Architecture Search}

%DARTS \citep{liu2019darts} searches for a computation cell as a building block of the final architecture. 
Differentiable architecture search (DARTS)~\citep{liu2019darts} relaxes the discrete architecture space by assigning continuous architectural parameters to every operation choice in that space. Typically, the search is done for a cell (e.g., convolutional or recurrent) which is stacked in a repetitive manner to form the full network. The cell itself is represented as a directed acyclic graph (DAG) with an ordered sequence of $N$ nodes. Every node $x^{(i)}$ denotes a latent representation and each edge $(i, j)$ is associated with an operation $o^{(i,j)} \in \gO$ that transforms $x^{(i)}$, where $\gO$ is a pre-defined space of operations. 
%A cell takes two inputs: outputs of the two previous cells and has one output. The output of the cell is obtained by applying a reduction operation to all the intermediate nodes.

The goal is to choose one operation from $\gO$ to connect each pair of nodes. 
%To make the search space differentiable, 
DARTS continuously relaxes these discrete choices by creating a convex combination of the operations in  $\gO$ using the mixed operation $\bar{o}$: 
\begin{equation}
    \bar{o}^{(i,j)}(x) = \sum_{o \in \gO}{
        \frac{\exp(\alpha_o^{(i,j)})}{\sum_{o' \in \gO}{\exp(\alpha_{o'}^{(i,j)})}} o(x),
    }
    \label{eq:BG:mixed_ops}
\end{equation}
where $\alpha_o^{(i,j)}$ is the operation mixing weight. 
Thus, the problem of searching for the cell architecture boils down to learning a set of continuous variables $\alpha = \{\alpha^{(i,j)}\}$. This allows to formulate the NAS problem as a bi-level optimization problem:
\begin{equation*}
    \min_{\alpha}{\gL_{val}(w^*(\alpha), \alpha)}
    \quad
    \text{s.t.} \quad 
    w^*(\alpha) = \argmin_{w}{\gL_{train}(w, \alpha)}.
    \label{eq:BG:darts_bi}
\end{equation*}
After the search, 
%the operation with the largest $\alpha^{(i,j)}_o$ is preserved for each edge. 
the final architecture is derived by retaining the top-$k$ strongest operations from all the previous nodes.

In our work, we use three efficient variations of DARTS, namely:

\textbf{PC-DARTS} \citep{xu2019pc} introduces partial channel connections, where only a portion of channels are sent to the mixed operation.
To overcome the instability induced by sampling, it introduces edge weights, $\beta$, explicitly for every edge. The connectivity of an edge is then determined by combining both $\alpha$ and $\beta$.

\textbf{DrNAS} \citep{chen2021drnas} 
%formulates DARTS as a distribution learning problem, where 
samples the $\alpha$ parameters from a parameterized Dirichlet distribution. 
Since it uses partial channel connections, it introduces a multi-stage scheme that increases the channel fraction while pruning the number of operators at every stage.

\textbf{RandomNAS} \citep{li2020random} builds a supernetwork similar to DARTS and simply uses randomly sampled architectures to train the shared weights during every mini-batch iteration. 
The trained shared weights are then used to evaluate the performance of multiple randomly sampled configurations and select the best performing one as the final architecture.

% --------------------------------------------------------------------

\section{NAS for multi-headed models}
% \tct{Maybe mention that the dimensions of alphas is different.}
\subsection{Search Space}

\begin{figure}
    \centering
    \includegraphics[width=0.7\linewidth]{figures/head_arch.pdf}
    \caption{Single-headed network from the search space}
    \label{fig:AP:head_arch}
\end{figure}

Similar to the DARTS search space \citep{liu2019darts}, we use a cell-based architecture for every head, as shown in Figure \ref{fig:AP:head_arch}. A head is made of $L$ cells, with the first cell as a reduction cell (reducing spatial dimensions) and the remaining $L-1$ as normal cells (keeping spatial dimensions).
Unlike DARTS, we do not distinguish the configurations between reduction and normal cells. We found that having different configurations for reduction and normal cells had little to no impact in the performance of a multi-headed ensemble and only expanded the architecture space. 
Hence, in a multi-head ensemble with $M$ heads, there are $M \times L$ cells but only $M$ cell configurations or $M \times \{\alpha\}$ parameters to optimize.

\subsection{Diversity Encouraging Loss for Differentiable Search}
% \tct{Did you show that this diversity term helps? Can't find the numbers.}

During the search phase of DARTS, there is no guarantee that the head architectures learnt via gradient descent would be diverse.
To this end, we introduce an additional diversity term only in the loss function for the architecture weights, $\gL_{val}$.
This ensures that the diversity in the one-shot model predictions originates from the architecture weights and not from the network weights.

We use the Jensen-Shannon Divergence (JSD) to measure the diversity between the individual head predictions and maximize it in the validation objective.
Unlike KL divergence, JSD is symmetric and bounded \citep{lin1991divergence}, which allows for direct maximization without the loss exploding.

Given $M$ heads, the diversity-encouraging loss term is:
\begin{align*}
    \gL_{jsd} &= JSD[f_{\theta_1}(x),...,f_{\theta_M}(x)] \\
            &= \frac{1}{M} \sum_{i=0}^{M}{
        KL[F(x) \parallel f_{\theta_i}(x)]
    } \\
    \gL_{val} &= \gL_{train} - \lambda_{jsd} \gL_{jsd}
    \label{eq:AP:archjsd}
\end{align*}

where $\lambda_{jsd}$ is the weight of the JSD loss. Refer to Appendix \ref{appendix:ablation} for ablations.
% \tct{The results in appendix do not show if the diversity term helps (in terms of final accuracy) or did I miss something?}
% \todo[inline]{FH: I don't understand the last line; this would say that the validation loss is always dominated by the training loss, since $\gL_{jsd}$ can't get negative, can it!? }
% \todo[inline]{AN: We maximize the JSD term in $\gL_{val}$ to increase the diversity in predictions. $\gL_{train}$ (cross entropy) dominates the term here as we still need to minimize $\gL_{val}$ to determine the arch. weights in the end. The diversity term only helps in "ensuring" that the predictions are not too similar.}
% --------------------------------------------------------------------

\section{Experiments} 

\subsection{Setup}
\textbf{Backbone architecture.} We use a WideResNet-40-2 \citep{zagoruyko2017wide} backbone for all the methods. The final block is then replaced with 3 cells from our search space.

\textbf{Baselines.} We compare our multi-headed ensemble methods with deep ensembles \citep{lakshminarayanan2016simple} (DeepEns (Sample) and DeepEns (RS)), NES-RS \citep{zaidi2020neural} and hyper-deep ensembles \citep{wenzel2021hyperparameter} (HyperDeepEns (RS)) from our search space. \textit{Sample} and \textit{RS} refer to head configurations that are randomly sampled and found by random search, respectively. We ran RS for 25 iterations (function evaluations). 

\textbf{Evaluation.} We compare the methods on NLL, classification error and ECE \citep{guo2017calibration}. All results are aggregates of 3 runs. We provide more details on the experimental setup in Appendix \ref{appendix:exp_details}. 

%\subsection{Performance Comparison}
\subsection{Results}

Figure \ref{fig:EX:ens_perf} shows the performance comparison of the ensemble methods on CIFAR-100 and Tiny-ImageNet for an ensemble size $M=3$. Figure \ref{fig:EX:ens_cost_c100} shows a comparison between the computational cost and ensemble performance.

\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{figures/ens_all_n3.pdf}
    \caption{Ensemble performance comparison for $M=3$ (mean $\pm$ std.dev.). M is the number of ensemble members or prediction heads.
    % \tct{Why does ECE increase with ensemble size? Seems like a general problem with larger ensembles. Is this behaviour known? I would suggest moving M=5 to supplementary if we do not have a good argument for why this is the case.}
    }
    \label{fig:EX:ens_perf}
\end{figure}

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.75\linewidth]{figures/cifar100/ens_cost_plot.pdf}
    \caption{Ensemble error  vs search cost (for $M=3$) on CIFAR-100. Data points closer to the origin are better. Size of each point is proportional to the final ensemble's model size.}
    \label{fig:EX:ens_cost_c100}
\end{figure}


As we can see, almost all multi-headed ensembles (even a randomly sampled configuration) show better uncertainty calibration than a deep ensemble.
% \todo[inline]{FH: hmm, I don't see that in Figure 3. For CIFAR-100, DeepEns(RS) actually has the \emph{overall lowest} ensemble error. Let's make this statement only about ECE.}
%Multi-headed ensembles are comparably or better calibrated than deep ensembles, both naive and configurations identified by ensemble search methods.
% Searching for a deep ensemble leads to the best ensemble performance on classification error.
Compared to NES and DeepEns (RS), the one-shot multi-headed search methods, especially DrNAS and RandomNAS, achieve comparable predictive performance, while being 3$\times$ more efficient during search.
% \todo[inline]{FH: Do I see it right in the figure that concerning ECE as an objective, NES-RS works performs very poorly? Do we know why that is? (In the NES paper, it was always better than DeepEns / HyperDeepEns.)} 
% \todo[inline]{AN: NES-RS performs poorer than expected because of this cell search space with a backbone. Deep ensembles from this space even had increasing model calibration with increasing ensemble sizes (Figure \ref{fig:appendix:mhe_vs_ind}), which was not the case for default WideResNet deep ensembles.}
Among the multi-headed methods, configurations identified by DrNAS perform the best in terms of prediction error. 
This can be attributed to the natural exploration-exploitation trade-offs in distribution learning. 
% \todo{FH: Hmm, again I'm confused: DrNAS actually performed very poorly concerning ECE, the worst among the MHE methods, no?}
% PC-DARTS however struggles to find good configurations that can outperform randomly samples from the search space.
RandomNAS also performed almost as well for small ensembles and for CIFAR-100 identified better configurations than a naive and expensive random search.

Interestingly, for larger ensemble sizes the performance of differentiable methods deteriorates while methods based on random search achieve better performance (Appendix \ref{appendix:ens_perf}). 
%Why do methods based on random search perform better than gradient-based NAS methods? 
%We explore this question further in the following section.
We provide more insights into this behavior in the following section.

\subsection{Analysis of Differentiable Search Methods}
\label{EX:darts_analysis}

%Since differentiable search methods have been providing state of the art neural architecture search performance in recent years while maintaining computational efficiency, we naturally expect them to provide competitive search performance here. 
\citet{zela2020understanding} demonstrated that DARTS can often find degenerate architectures depending on the search space at hand.
%However, the results we found were surprising as the differentiable search methods
Similarly, we found that PC-DARTS and DrNAS struggled to find architectures better than random search, or even random \emph{samples}, especially for larger ensemble sizes.

A Hessian norm analysis of $\nabla^2\gL_{valid}$ \citep{zela2020understanding} of these methods (Appendix \ref{appendix:darts_analysis}) indicated that this was not attributed to architecture over-fitting in the one-shot model: both PC-DARTS and DrNAS were able to find well performing configurations for a single network from the search space, though not for the multi-headed space.

\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{figures/cifar100/rs_var_and_regret.pdf}
    \caption{\textit{(left)} Distribution of validation NLL from 60 samples across 3 random search runs. \textit{(right)} Validation NLL Regret from optimal configuration of random search (mean $\pm$ std.dev.). All results on CIFAR-100.}
    \label{fig:EX:head_variance_c100}
\end{figure}

To this end, we analyze the search space by randomly sampling configurations for different ensemble sizes. Figure \ref{fig:EX:head_variance_c100} shows that while there is a clear improvement in the mean ensemble performance when scaling up the number of heads, the variance in the ensemble performance decreases significantly.
The validation regret curves flatten out with more heads, 
%further indicate that the loss landscape becomes flatter, 
% \todo[inline]{FH: How do they indicate this? It could also just indicate that RS doesn't find better solutions.}
% \todo[inline]{AN: Yes, it could also mean that RS cannot find better configurations. But the reduced variance in the performance of sampled configurations indirectly leads to flatter regret curves. I included the t-SNE visualization in appendix (Figure \ref{fig:EX:arch_surface}) to show the distribution of losses across the search space, can that work?}
indicating that diminishing returns can be expected for running a more complex search method for $M > 5$ (while increasing computational demands).
%, any search method will only provide minimal improvement, while being computationally more expensive. 
A similar behaviour can be observed on Tiny-ImageNet in Appendix \ref{appendix:darts_analysis}.

Furthermore, 
%these differentiable methods search for only 2 cells in most previous works
while most NAS methods previously searched for only 2 cells~\citep{liu2019darts, zhou2019bayesnas, xu2019pc, chen2021drnas}, our search space size increases exponentially with the number of ensemble members/heads. We hypothesize that this, coupled with a low variance regime, leads the DARTS-based methods to get stuck in local optima and find suboptimal configurations.
This could also explain why random search traverses the operation search space better and identifies better performing configurations.

% --------------------------------------------------------------------

\section{Conclusion and Future Work} 

%We introduced a search space for multi-headed architectures and performed one-shot neural architecture search to construct robust  ensembles.
In this work, we introduced a method for efficiently searching for the architectures of the individual heads in a multi-headed ensemble.
%that have reduced training costs.
%We demonstrated lower search costs compared to other ensemble search methods.
%We demonstrated that one-shot search is significantly more efficient than searching for a deep ensemble. 
%Under memory and time constraints, multi-headed ensembles can 
The resulting models are accurate, well calibrated and also more efficient (computationally and memory-wise) compared to deep ensembles and other methods found using inefficient methods that require training every ensemble base learner individually. 
%In the future, we would like to understand why random search based approaches work so well for ensembles.
%In the future, we would also like to investigate further why gradient-based approaches perform sub-optimally in the multi-headed setting. 
In the future, we would like to improve the robustness of differentiable NAS methods applied to ensemble learning.
%they still are some of the most efficient NAS methods available. 


==> Multihead NES/figures/cifar100/ens_cost.tex <==
\begin{table}[ht]
    \centering
    \caption{Performance and computation cost of different search methods for ensemble size $M=3$ on CIFAR-100.
    % \tct{I think latency is more commonly used than evaluation time. Latency - compute forward propagation time on the same GPU multiple times and take the mean. Ignore dataloading time.}
    }
    \vspace{2mm}
	{%\scriptsize
	\resizebox{1.0\linewidth}{!}{
	\begin{tabular}{lcccc}
	\toprule
	\textbf{Method} & \textbf{\# Params} & \textbf{Search} & \textbf{Error} & \textbf{ECE} \\
					& \textbf{(M)}       & \textbf{(GPU hours)} & & \\
	\midrule
	DeepEns (Sample) & 4.1 & & 20.52\tiny{$\pm$0.12} & 0.019\tiny{$\pm$0.001} \\
	DeepEns (RS) & 4.2 & 15.2 & 19.58\tiny{$\pm$0.03} & 0.018\tiny{$\pm$0.001} \\
	HyperDeepEns (RS) & 4.2 & 28.7 & 20.11\tiny{$\pm$0.18} & 0.019\tiny{$\pm$0.003} \\
	NES-RS & 4.0 & 15.2 & 19.75\tiny{$\pm$0.27} & 0.021\tiny{$\pm$0.001} \\
	MHE-RS & 2.4 & 27.2 & 20.03\tiny{$\pm$0.12} & 0.015\tiny{$\pm$0.001} \\
	MHE (PC-DARTS) & 2.6 & 5.8 & 20.23\tiny{$\pm$0.04} & 0.017\tiny{$\pm$0.002} \\
	MHE (DrNAS) & 2.7 & 5.0 & 19.65\tiny{$\pm$0.09} & 0.017\tiny{$\pm$0.001} \\
	MHE (RandomNAS) & 2.6 & 8.1 & 19.86\tiny{$\pm$0.08} & 0.015\tiny{$\pm$0.001} \\
	\bottomrule
	\end{tabular}
	}
	}
    \label{tab:EX:ens_cost}
\end{table}


==> Multihead NES/figures/cifar100/ens_perf_cost_m3_40_2.tex <==
\begin{tabular}{ccccccccc}
\toprule
\textbf{Method} & \multicolumn{2}{c}{\textbf{Clean Performance}} & \multicolumn{2}{c}{\textbf{Corruption Performance}} &           \textbf{Params (M)} & \multicolumn{2}{c}{\textbf{Train Time (GPU hours)}} \\
         &         \textbf{Error(\%)} &            \textbf{ECE} &              \textbf{Error(\%)} &            \textbf{ECE}            &  & \textbf{Search} & \textbf{Evaluation} \\
\midrule
DeepEns &      20.81\tiny{$\pm$0.12} &  0.026\tiny{$\pm$0.001} &           49.74\tiny{$\pm$0.10} &  0.155\tiny{$\pm$0.001}          & 6.8 & & 1.4 \\
DeepEns (Sample) &      20.52\tiny{$\pm$0.19} &  0.019\tiny{$\pm$0.001} &           48.57\tiny{$\pm$0.08} &  0.114\tiny{$\pm$0.001}          & 4.1 & & 2.2 \\
DeepEns (RS) &      19.58\tiny{$\pm$0.03} &  0.018\tiny{$\pm$0.001} &           47.22\tiny{$\pm$0.10} &  0.090\tiny{$\pm$0.000}           & 4.2 & 15.2 & 2.3 \\
HyperDeepEns &      20.94\tiny{$\pm$0.06} &  0.020\tiny{$\pm$0.004} &           49.24\tiny{$\pm$0.03} &  0.112\tiny{$\pm$0.000}           & 6.8 & 13.5 & 1.4 \\
HyperDeepEns (RS) &      20.11\tiny{$\pm$0.18} &  0.021\tiny{$\pm$0.003} &           47.91\tiny{$\pm$0.13} &  0.149\tiny{$\pm$0.002}            & 4.2 & 28.7 & 2.3 \\
NES-RS &      19.75\tiny{$\pm$0.27} &  0.021\tiny{$\pm$0.001} &           48.13\tiny{$\pm$0.35} &  0.099\tiny{$\pm$0.004}           & 4.0 & 15.2 & 2.2 \\
ONE &      20.31\tiny{$\pm$0.21} &  0.043\tiny{$\pm$0.003} &           49.39\tiny{$\pm$0.07} &  0.184\tiny{$\pm$0.003}           & 5.7 & & 0.7 \\
MHE-Sample &      20.21\tiny{$\pm$0.08} &  0.018\tiny{$\pm$0.001} &           48.93\tiny{$\pm$0.44} &  0.131\tiny{$\pm$0.008}          & 2.4 & & 1.2 \\
MHE-RS &      20.03\tiny{$\pm$0.12} &  0.015\tiny{$\pm$0.001} &           49.16\tiny{$\pm$0.17} &  0.133\tiny{$\pm$0.004}           & 2.6 & 27.2 & 1.3 \\
MHE-PCD &      20.23\tiny{$\pm$0.04} &  0.017\tiny{$\pm$0.002} &           47.81\tiny{$\pm$0.16} &  0.110\tiny{$\pm$0.004}          & 2.7 & 5.8 & 1.3 \\
MHE-DRN &      19.65\tiny{$\pm$0.09} &  0.017\tiny{$\pm$0.001} &           47.85\tiny{$\pm$0.28} &  0.113\tiny{$\pm$0.005}          & 2.7 & 5.0 & 1.3 \\
MHE-RNAS &      19.86\tiny{$\pm$0.08} &  0.015\tiny{$\pm$0.001} &           48.55\tiny{$\pm$0.33} &  0.124\tiny{$\pm$0.005}            & 2.6 & 8.1 & 1.3 \\
\bottomrule
\end{tabular}


==> Multihead NES/figures/cifar100/perf_m1.tex <==
\begin{table}[ht]
    \centering
    \caption{Performance of different search methods for one head on CIFAR-100 dataset. WideResNet block is the baseline block used in the original network.}
    
    {\scriptsize
    \begin{tabular}{ccc}
    \toprule
    \textbf{Method} & \textbf{NLL} & \textbf{Error} \\
    \midrule
    WideResNet block & 1.089\tiny{$\pm$0.006} & 24.41\tiny{$\pm$0.08} \\
    Random Sample & 0.983\tiny{$\pm$0.020} & 24.12\tiny{$\pm$0.21} \\
    Random Search & 0.927\tiny{$\pm$0.015} & \best{23.17}\tiny{$\pm$0.08} \\
    PC-DARTS & 0.923\tiny{$\pm$0.008} & \best{23.20}\tiny{$\pm$0.10} \\
    DrNAS & \best{0.908}\tiny{$\pm$0.007} & 23.61\tiny{$\pm$0.21} \\
    \bottomrule
    \end{tabular}
    }
    \label{tab:EX:perf_m1}
\end{table}

==> Multihead NES/figures/tinyim/ens_perf_cost_m3_40_2.tex <==
\begin{tabular}{cccccc}
\toprule
\textbf{Method} & \multicolumn{2}{c}{\textbf{Clean Performance}} & \multicolumn{2}{c}{\textbf{Corruption Performance}} \\
         &         \textbf{Error(\%)} &            \textbf{ECE} &              \textbf{Error(\%)} &            \textbf{ECE} \\
\midrule
DeepEns &      34.96\tiny{$\pm$0.08} &  0.030\tiny{$\pm$0.002} &           72.51\tiny{$\pm$0.15} &  0.168\tiny{$\pm$0.001} \\
DeepEns (Sample) &      34.54\tiny{$\pm$0.18} &  0.024\tiny{$\pm$0.003} &           73.15\tiny{$\pm$0.08} &  0.156\tiny{$\pm$0.001} \\
DeepEns (RS) &      33.44\tiny{$\pm$0.19} &  0.023\tiny{$\pm$0.001} &           71.46\tiny{$\pm$0.05} &  0.121\tiny{$\pm$0.002} \\
HyperDeepEns &      35.39\tiny{$\pm$0.42} &  0.049\tiny{$\pm$0.004} &           72.63\tiny{$\pm$0.22} &  0.119\tiny{$\pm$0.001} \\
HyperDeepEns (RS) &      33.57\tiny{$\pm$0.08} &  0.072\tiny{$\pm$0.005} &           71.99\tiny{$\pm$0.10} &  0.081\tiny{$\pm$0.003} \\
NES-RS &      33.17\tiny{$\pm$0.23} &  0.038\tiny{$\pm$0.002} &           71.53\tiny{$\pm$0.12} &  0.132\tiny{$\pm$0.002} \\
ONE &      34.39\tiny{$\pm$0.12} &  0.029\tiny{$\pm$0.001} &           71.78\tiny{$\pm$0.06} &  0.184\tiny{$\pm$0.002} \\
MHE-Sample &      33.81\tiny{$\pm$0.15} &  0.022\tiny{$\pm$0.002} &           71.78\tiny{$\pm$0.17} &  0.162\tiny{$\pm$0.002} \\
MHE-RS &      33.75\tiny{$\pm$0.24} &  0.023\tiny{$\pm$0.002} &           71.60\tiny{$\pm$0.33} &  0.151\tiny{$\pm$0.003} \\
MHE-PCD &      34.17\tiny{$\pm$0.31} &  0.022\tiny{$\pm$0.002} &           73.17\tiny{$\pm$0.33} &  0.171\tiny{$\pm$0.001} \\
MHE-DRN &      33.55\tiny{$\pm$0.55} &  0.030\tiny{$\pm$0.004} &           71.24\tiny{$\pm$0.37} &  0.168\tiny{$\pm$0.004} \\
MHE-RNAS &      33.46\tiny{$\pm$0.19} &  0.024\tiny{$\pm$0.004} &           72.17\tiny{$\pm$0.21} &  0.161\tiny{$\pm$0.002} \\
\bottomrule
\end{tabular}


==> Multihead NES/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> Multihead NES/setup.tex <==
\usepackage{subcaption}
\usepackage{xcolor}
\usepackage{todonotes}
\newcommand{\denselist}{\itemsep 0pt\topsep-6pt\partopsep-6pt}

\input{math_commands}

\definecolor{cadmiumgreen}{rgb}{0.0, 0.42, 0.24}

\newcommand{\tct}[1]{\textcolor{cadmiumgreen}{ #1}} % Tonmoy's comments

\newcommand{\best}[1]{\textbf{#1}}
\newcommand{\mine}[1]{\underline{#1}}
\newcommand{\both}[1]{\textbf{\underline{#1}}}


==> figures/cifar100/ens_perf_cost_m3_40_2.tex <==
\begin{tabular}{ccccccccc}
\toprule
\textbf{Method} & \multicolumn{2}{c}{\textbf{Clean Performance}} & \multicolumn{2}{c}{\textbf{Corruption Performance}} &           \textbf{Params (M)} & \multicolumn{2}{c}{\textbf{Train Time (GPU hours)}} \\
         &         \textbf{Error(\%)} &            \textbf{ECE} &              \textbf{Error(\%)} &            \textbf{ECE}            &  & \textbf{Search} & \textbf{Evaluation} \\
\midrule
DeepEns &      20.81\tiny{$\pm$0.12} &  0.026\tiny{$\pm$0.001} &           49.74\tiny{$\pm$0.10} &  0.155\tiny{$\pm$0.001}          & 6.8 & & 1.4 \\
DeepEns (Sample) &      20.52\tiny{$\pm$0.19} &  0.019\tiny{$\pm$0.001} &           48.57\tiny{$\pm$0.08} &  0.114\tiny{$\pm$0.001}          & 4.1 & & 2.2 \\
DeepEns (RS) &      19.58\tiny{$\pm$0.03} &  0.018\tiny{$\pm$0.001} &           47.22\tiny{$\pm$0.10} &  0.090\tiny{$\pm$0.000}           & 4.2 & 15.2 & 2.3 \\
HyperDeepEns &      20.94\tiny{$\pm$0.06} &  0.020\tiny{$\pm$0.004} &           49.24\tiny{$\pm$0.03} &  0.112\tiny{$\pm$0.000}           & 6.8 & 13.5 & 1.4 \\
HyperDeepEns (RS) &      20.11\tiny{$\pm$0.18} &  0.021\tiny{$\pm$0.003} &           47.91\tiny{$\pm$0.13} &  0.149\tiny{$\pm$0.002}            & 4.2 & 28.7 & 2.3 \\
NES-RS &      19.75\tiny{$\pm$0.27} &  0.021\tiny{$\pm$0.001} &           48.13\tiny{$\pm$0.35} &  0.099\tiny{$\pm$0.004}           & 4.0 & 15.2 & 2.2 \\
ONE &      20.31\tiny{$\pm$0.21} &  0.043\tiny{$\pm$0.003} &           49.39\tiny{$\pm$0.07} &  0.184\tiny{$\pm$0.003}           & 5.7 & & 0.7 \\
MHE-Sample &      20.21\tiny{$\pm$0.08} &  0.018\tiny{$\pm$0.001} &           48.93\tiny{$\pm$0.44} &  0.131\tiny{$\pm$0.008}          & 2.4 & & 1.2 \\
MHE-RS &      20.03\tiny{$\pm$0.12} &  0.015\tiny{$\pm$0.001} &           49.16\tiny{$\pm$0.17} &  0.133\tiny{$\pm$0.004}           & 2.6 & 27.2 & 1.3 \\
MHE-PCD &      20.23\tiny{$\pm$0.04} &  0.017\tiny{$\pm$0.002} &           47.81\tiny{$\pm$0.16} &  0.110\tiny{$\pm$0.004}          & 2.7 & 5.8 & 1.3 \\
MHE-DRN &      19.65\tiny{$\pm$0.09} &  0.017\tiny{$\pm$0.001} &           47.85\tiny{$\pm$0.28} &  0.113\tiny{$\pm$0.005}          & 2.7 & 5.0 & 1.3 \\
MHE-RNAS &      19.86\tiny{$\pm$0.08} &  0.015\tiny{$\pm$0.001} &           48.55\tiny{$\pm$0.33} &  0.124\tiny{$\pm$0.005}            & 2.6 & 8.1 & 1.3 \\
\bottomrule
\end{tabular}


==> figures/tinyim/ens_perf_cost_m3_40_2.tex <==
\begin{tabular}{cccccc}
\toprule
\textbf{Method} & \multicolumn{2}{c}{\textbf{Clean Performance}} & \multicolumn{2}{c}{\textbf{Corruption Performance}} \\
         &         \textbf{Error(\%)} &            \textbf{ECE} &              \textbf{Error(\%)} &            \textbf{ECE} \\
\midrule
DeepEns &      34.96\tiny{$\pm$0.08} &  0.030\tiny{$\pm$0.002} &           72.51\tiny{$\pm$0.15} &  0.168\tiny{$\pm$0.001} \\
DeepEns (Sample) &      34.54\tiny{$\pm$0.18} &  0.024\tiny{$\pm$0.003} &           73.15\tiny{$\pm$0.08} &  0.156\tiny{$\pm$0.001} \\
DeepEns (RS) &      33.44\tiny{$\pm$0.19} &  0.023\tiny{$\pm$0.001} &           71.46\tiny{$\pm$0.05} &  0.121\tiny{$\pm$0.002} \\
HyperDeepEns &      35.39\tiny{$\pm$0.42} &  0.049\tiny{$\pm$0.004} &           72.63\tiny{$\pm$0.22} &  0.119\tiny{$\pm$0.001} \\
HyperDeepEns (RS) &      33.57\tiny{$\pm$0.08} &  0.072\tiny{$\pm$0.005} &           71.99\tiny{$\pm$0.10} &  0.081\tiny{$\pm$0.003} \\
NES-RS &      33.17\tiny{$\pm$0.23} &  0.038\tiny{$\pm$0.002} &           71.53\tiny{$\pm$0.12} &  0.132\tiny{$\pm$0.002} \\
ONE &      34.39\tiny{$\pm$0.12} &  0.029\tiny{$\pm$0.001} &           71.78\tiny{$\pm$0.06} &  0.184\tiny{$\pm$0.002} \\
MHE-Sample &      33.81\tiny{$\pm$0.15} &  0.022\tiny{$\pm$0.002} &           71.78\tiny{$\pm$0.17} &  0.162\tiny{$\pm$0.002} \\
MHE-RS &      33.75\tiny{$\pm$0.24} &  0.023\tiny{$\pm$0.002} &           71.60\tiny{$\pm$0.33} &  0.151\tiny{$\pm$0.003} \\
MHE-PCD &      34.17\tiny{$\pm$0.31} &  0.022\tiny{$\pm$0.002} &           73.17\tiny{$\pm$0.33} &  0.171\tiny{$\pm$0.001} \\
MHE-DRN &      33.55\tiny{$\pm$0.55} &  0.030\tiny{$\pm$0.004} &           71.24\tiny{$\pm$0.37} &  0.168\tiny{$\pm$0.004} \\
MHE-RNAS &      33.46\tiny{$\pm$0.19} &  0.024\tiny{$\pm$0.004} &           72.17\tiny{$\pm$0.21} &  0.161\tiny{$\pm$0.002} \\
\bottomrule
\end{tabular}

